Towards a Methodology for Participant Selection in Software Engineering Experiments. A Vision of the Future

Background. Software Engineering (SE) researchers extensively perform experiments with human subjects. Well-defined samples are required to ensure external validity. Samples are selected \textit{purposely} or by \textit{convenience}, limiting the generalizability of results. Objective. We aim to depict the current status of participants selection in empirical SE, identifying the main threats and how they are mitigated. We draft a robust approach to participants' selection. Method. We reviewed existing participants' selection guidelines in SE, and performed a preliminary literature review to find out how participants' selection is conducted in SE in practice. % and 3) we summarized the main issues identified. Results. We outline a new selection methodology, by 1) defining the characteristics of the desired population, 2) locating possible sources of sampling available for researchers, and 3) identifying and reducing the "distance" between the selected sample and its corresponding population. Conclusion. We propose a roadmap to develop and empirically validate the selection methodology.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> sections/StatePractice.tex <==
\section{State of the Practice}
\label{sec:statePractice}

\df{We should merge Section 2: State of Practice and Section 4 Related Work. The final message of this section should be that---as a community---we do not have an agreement on what are the dimensions to be used for participants selection (the existing one, students vs. professional, is unsatisfactory). }\\
\od{Let's wait until wee see the substance in the related work section}

\subsection{Search and Selection Process and Data Extraction}
We systematically collected papers in the recommended source engines for Systematic Literature Review \footnote{We adopted the weight source engines recommended by the Systematic Literature Review (SLR) guideline: ACM Digital Library, IEEEXplore Digital Library, Science Direct, Scopus, Google Scholar, CiteSeer library, Inspec, Springer link.} that conducted controlled experiments in software engineering. 
% \sv{@Valentina, where commonly SE experiments are published? (is this what you mean?)}.
As search string we used: ``\textit{controlled experiment*}'' OR ``\textit{controlled-experiment*}''. We applied this string on title and abstract. 
% \sv{@Valentina, where? Title/abstract?}.
We decided to concentrate only on the papers published in the last five years (2017-2021), retrieving 118 unique papers \footnote{the rawdata are available here: LINK}
For each paper, we checked two important aspects: 1) the strategy adopted for the participant's selection and 2) the identified threats to validity. 

% \sv{@Valentina, do all papers report a single experiment? More than one? If so, perhaps it makes sense to clarify. Of course it could be that all experiments in the same paper use the same participants...}\\
% \va{@Sira: single experiment}

\subsection{Results}
\textbf{Participants selection strategy:} The vast majority of the considered studies (90 studies) selected the participants based on the current availability at the moment of the study. While the remaining studies did not report any details about the selection. 

In case of bachelor or master students, the authors selected them from the related course closer to the topic of the study. 
In other cases, the authors selected the participants based on the latter experience in the study context, such as programming languages.

Whether participants characteristics are taken into consideration, the authors simply tested their experience in the domain profiling the background skills via preliminary surveys in case of industrial participants.

% \sv{@Valentina, What does this mean? Define and provide examples}. 

% \sv{@Valentina, this does not seem participants selection strategy. Do they simply test or select based on the test? Perhaps this is a third aspect? Whether participants characteristics are taken into consideration.} 

% Only a few study (only 2 studies) adopted more sophisticated strategy such as convenience sampling to recruit participants for the experiment.

% \sv{@Valentina, isn´t convnience sampling the same as current availability?}

% \vspace{2mm}
\textbf{Threats to validity for participant selection:} in 50 studies, the authors reported to be aware of the limitations of the participants selection. However, they did not discuss possible mitigation actions for this threat.

% \sv{@Valentina, what is the meaning of in depth?}. 


\subsection{Discussion/Implications}
We found two studies that characterize and discuss the strategies adopted in the participants selection process~\cite{amir2018there,SHH05}. 

Amir and Ralph~\cite{amir2018there} investigated 236 papers published at EMSE between 2012 and 2016.
They show that actual random sampling is rare (only 3\% of the studies), whereas purposive (i.e., create a sample based on a strategy) and convenience (i.e., create a sample arbitrarily) sampling are dominant and stable over time. 
The authors attribute the lack of random sampling to the lack of well-defined sampling frames from which elements can be selected\footnote{Another assumption is that a random sampling strategy will result in a representative bias. For an in depth explanation of why this reasoning is flawed, we refer to \cite{baltes2020sampling, amir2018there}.}.

\sv{How does purposive sample fit in the Related Work section? It should correspond to any of the things we mention...}

Purposive sampling is the dominant strategy in SE experiments also according to a review of the literature by Baltes and Raph~\cite{baltes2020sampling} which includes 115 empirical studies published between 2014 and 2019 at the International Conference on Software Engineering (ICSE),  ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering (ESEC/FSE), Transaction in Software Engineering (TSE), and Transaction in Software Engineering and Methodology (TOSEM). 
The authors show that purposive sampling and random sampling are respectively used in 77\% and 4\% of the experiments.
Other sampling techniques, stratified sampling is used in 1\% of the experiments whereas snowballing is not used at all.

Sj\o berg \textit{et al.} review shows that only two (out of 103) primary studies claim random sampling, but how it was carried out was not reported~\cite{SHH05}. 
The majority of the experiments use convenience sampling, with students being the most used type of participants~\cite{SHH05}.
The authors recommend to incentivize professionals to be part of experimental samples, for example, by compensating employers for the hours their personnel spent on a study, as well as offer workshops to the companies where assessments are used as experimental session~\cite{SHH05,vegas2015difficulties}.

==> sections/TheRoadMap.tex <==
\section{The RoadMap}
\label{sec:roadmap}



==> sections/UnusedText.tex <==

\subsection*{Possible candidates for interviewing}

\begin{itemize}
    \item Natalia Juristo
    \item Marcela Genero, because she has run two families of experiments at least, if I am not wrong.
    \item Who else, and why? Please add candidates here
\end{itemize}

